Omnimatte: Associating Objects and Their Effects in Video

Computer vision is increasingly effective at segmenting objects in images and videos; however, scene effects related to the objects -- shadows, reflections, generated smoke, etc -- are typically overlooked. Identifying such scene effects and associating them with the objects producing them is important for improving our fundamental understanding of visual scenes, and can also assist a variety of applications such as removing, duplicating, or enhancing objects in video. In this work, we take a step towards solving this novel problem of automatically associating objects with their effects in video. Given an ordinary video and a rough segmentation mask over time of one or more subjects of interest, we estimate an omnimatte for each subject -- an alpha matte and color image that includes the subject along with all its related time-varying scene elements. Our model is trained only on the input video in a self-supervised manner, without any manual labels, and is generic -- it produces omnimattes automatically for arbitrary objects and a variety of effects. We show results on real-world videos containing interactions between different types of subjects (cars, animals, people) and complex effects, ranging from semi-transparent elements such as smoke and reflections, to fully opaque effects such as objects attached to the subject.

==> method_backup.tex <==
\section{Estimating Omnimattes from Video}
\label{sec:method}
The input to our method is an ordinary video of moving objects, and one or more layers of rough segmentation masks that mark the subjects of interest.
The output is an \emph{omnimatte} for each input mask layer, consisting of an alpha matte (opacity map) and a color image. We additionally produce a color background layer containing the static background elements. The model is trained to reconstruct the test video without observing any additional examples, in a self-supervised manner. 



To accurately reconstruct the full video the model must infer all the time-varying scene elements from the input layers. 
Our goal is to steer the model to place the associated effects in the layer of the subject causing them. Lu, et al.~\cite{lu2020layered} showed that proper construction of the layer inputs will make the network favor predicting time-varying effects from the input corresponding to the object causing those effects. For example, the mask of the person in the video in Figure~\ref{fig:teaser} provides more information about its shadow compared with the mask of the dog, so the network tends to learn to predict the person's shadow from the person's mask. Our task is to design network inputs and losses that encourage this solution for general objects. Where Lu, et al.~\cite{lu2020layered} used an explicit human model for the network inputs, we use a general, flow-based model (Sec.~\ref{sec:training_overview}) and flow-based losses (Sec.~\ref{sec:flow_losses}). 


\tali{Can we change this to just Overview?}
\subsection{Training Overview}
\label{sec:training_overview}

Figure~\ref{fig:pipeline} illustrates our pipeline.  Our model processes the video in a frame by frame fashion, where the architecture is a 2D U-Net.  For each frame, we compute rough object masks using off-the-shelf techniques to mark the major moving objects in the scene. Based on the desired output, we group the objects into $N$ mask layers $\{M^t_i\}_{i=1}^N$ and define a (possibly time-varying) ordering $o_t$ for the layers. For example, in a scene with a rider, a bicycle, and several people in a crowd, we might group the rider and bicycle into one layer, while grouping the crowd into a second layer. To equip our model with explicit information about \emph{object motion} and frame-to-frame correspondence, we also compute a dense optical flow field, $F^t$, between each frame and the consecutive frame in the video. We then mask this flow field by each of the input masks $M^t_i$ to provide the network only flow information related to the layer's subject.


From this rough yet explicit representation of moving objects, the model has to infer: (i) \emph{omnimattes} -- pairs of continuous-valued opacity maps (matte) and RGB images that capture not only the $i^{th}$ moving object but also all the scene elements that are correlated with it in space and time (e.g., reflections, shadows, attached objects, etc.), (ii) a refined optical flow field for each layer, and (iii) a background RGB images. Formally,

\begin{equation}
 \text{Omnimatte}(I_t, M_t^i, F_t^{i}) = \mathcal{L}_t = \{\alpha_t^i, C_t^i, \hat{F}^{i}_t\},   
\end{equation}
where $I_t$, $M_t^i$ and $F_t^i$ is the input video RGB frame, the initial input mask, and the pre-computed flow field of the $i^{th}$ object in time $t$, respectively. $\alpha^i_t$ and $C_t^i$ are the alpha and color buffers of the output omnimatte, and $\hat{F}^t_{i}$ is the predicted object flow. 





\subsection{RGBA Losses}
We apply several losses to the RGBA components of the output omnimattes. These losses are based on similar losses in~\cite{lu2020layered}. The main loss that drives our objective is a \emph{reconstruction loss}. Formally, we composite the set of estimated layers for each frame and  the predicted background layer using  standard back-to-front compositing, and encourage the composite image to match the original frame:
\begin{equation}
    \mathbf{E}_\text{rgb-recon} = \frac{1}{T}\sum_t \|I_t  - Comp(\mathcal{L}_t, o_t)\|_1,
    \label{eq:frame_recon}
\end{equation}
where $\mathcal{L}_t  = \{\alpha^i_t, C_t^i\}_{i=1}^N$ are the predicted layers for frame $t$, and $o_t$ is the compositing order that is assumed to be known.

To prevent a trivial solution where a single layer reconstruct the entire frame, we further apply a regularization loss to the $\alpha_t^i$ to encourage them to be spatially sparse. As in~\cite{lu2020layered}, we use a mix of $L_1$ and an approximate-$L_0$:
\begin{equation}
    \mathbf{E_{\mathtt{reg}}}  =  \frac{1}{T}\frac{1}{N}\sum_t \sum_i  \gamma \left \| \alpha_t^i \right \|_1 + \Phi_0(\alpha_t^i)
    \label{eq:matte_reg}
\end{equation}
where $\Phi_0(x) =  2\cdot \mathtt{Sigmoid}(5x) - 1$ smoothly penalizes non-zero values of the alpha map, and $\gamma$ controls the relative weight between the terms. 

Additionally, the reconstruction loss alone is not enough to guide the optimization to convergence from a random initialization. We therefore adopt a ``bootstrap'' loss to coerce the alpha maps $\alpha_t^i$ to match the input masks $M_t^i$:
\begin{equation}
    \mathbf{E}_\text{mask} = \frac{1}{T}\frac{1}{N}\sum_t \sum_i \left \| d_t^i \odot (M_t^i - \alpha_t^i) \right \|_2
\end{equation}
where $d_t^i = 1 - \mathtt{dilate}(M_t^i) + M_t^i$ is a boundary erosion mask to turn off the loss near the mask boundary, and $\odot$ is element-wise product.

\subsection{Flow Losses}
\label{sec:flow_losses}

Unlike~\cite{lu2020layered}, our model additionally predicts a set of \emph{flow layers}. Predicting flow layers serves as an auxiliary task that injects information about motion to our model and improves our decomposition (as demonstrated by our experiments). To achieve that we apply a \emph{flow reconstruction loss} and a \emph{photometric warping loss} defined below:
\begin{equation}
    \mathbf{E}_\text{flow-recon} = \frac{1}{T}\sum_t W_t \cdot \|F_t  - \textit{Comp}(\mathcal{F}_t, o_t)\|_1,
    \label{eq:frame_recon}
\end{equation}
where $\mathcal{F}_t = \{\hat{F}_i^t\}$ is the set of predicted flow layers, $F_t$ is the original, pre-computed flow, and $W_t$ is a spatial weighting map that lowers the impact of pixels with inaccurate flow.  Specifically, the confidence at each pixel $p$ is given by:
\begin{equation}
    W_t(p) =  W_{t}^{lr}(p) \cdot W_{t}^{p}(p) \cdot M_t(p),
\end{equation}

where $W_t^{lr}$ is computed using a standard left-right flow consistency error by: $W_t^{lr}(p) = \max (1-e_t^{lr}(p), 0)$, and $e_{lr}$ is the forward-backward flow error. $W_t^p$ measures photometric error and is given by: $W_t^p = \mathbbm{1}_{e_p<\beta}$, where $e_p = \|T(I_{t+1}; F_{t,t+1}) - I_t\|_1$ measures the photometric difference between $I_{t}$ and $I_{t+1}$ when backward warped using the flow. We set the threshold $\beta=20$. Finally, we mask the regions outside of the object mask $M_t$ since semi-transparent effects such as shadows tend to have inaccurate flow.

While the initial input flow is only available at the rough initial object region, the output flow layer should be valid in all areas that are visible from that layer (i.e., $\alpha^i_t > 0$). Such regions include complex regions for alignment such as shadows and reflections, and are likely to be discounted from the flow reconstruction loss.  We thus add a photometric data term to estimate the flow in those regions:

\begin{equation}
    \mathbf{E}_\text{photo} = \frac{1}{T}\sum_t \|I_t  - \textit{Comp}\left(\mathcal{L}_{wt}, \mathcal{F}_t\right), o_t)\|_1,
    \label{eq:warpping}
\end{equation}
where $\mathcal{L}_{wt}=\textit{Warp}(\mathcal{L}_{t+1}, \mathcal{F}_t)$ are the layers at time $t+1$ warped to time $t$ using the predicted flow layers. This is done for each layer separately, warping both the color image and the alpha matte. This loss also implicitly impose temporal coherency because the layer at time $t+1$ should explain the visual observation at time $t$.

We additionally encourage temporal consistency within layers using an \textit{alpha warping loss}:
\begin{equation}
    \mathbf{E}_\text{alpha-warp} = \frac{1}{T}\frac{1}{N}\sum_t \sum_i \|\alpha_t^i  - \alpha_{wt}^i\|_1,
    \label{eq:warpping}
\end{equation}

where $\alpha_{wt}^i = \textit{Warp}(\alpha_{t+1}^i, \mathcal{F}_t^i)$ is the predicted alpha for layer $i$ at time $t+1$ warped to time $t$ using the predicted flow.

\tali{I feel maybe this needs a figure: showing initial object flow in the rough mask, confidence map, and predicted flow, maybe showing that the initial flow does not align the shadow, but the predicted flow does?}

To conclude, our total loss is given by:
\begin{equation}
    \mathbf{E}_\text{frame-recon} + \lambda_\text{r} \mathbf{E}_\text{reg} +
    \lambda_\text{m} \mathbf{E}_\text{mask} + \\
    \mathbf{E}_\text{flow-recon} + \lambda_\text{p} \mathbf{E}_\text{photo} + \\
    \lambda_\text{w} \mathbf{E}_\text{alpha-warp},
\end{equation}
where $\lambda_\text{r} = .005, 
    \lambda_\text{m} = 50$ until $\mathbf{E}_\text{mask}$ falls below a threshold, and is $0$ afterward;
    $\lambda_\text{p} = 0.25$, and
    $\lambda_\text{w} = .005$.
 

\subsection{Camera-Aware Input Layers}
\tali{forrester, before we talk about camera motion, shouldn't we explain how a static background with a static camera can be estimated? I think we don't mention it before. Maybe it makes sense to merge this and the following section? first desr}
We assume the background scene is stationary and camera motion can be modeled by a time-varying homography from an unwrapped ``canvas'' image. The best-fitting homographies from frame $t$ to the canvas are found via feature tracking~\cite{grundmann2011auto} in a preprocess and are held fixed.

To make the network aware of the camera motion when rendering the foreground layers, the mask layers $M_t^i$ are augmented by compositing them over a texture image that tracks the camera. A random noise texture $\Bar{Z}$ is created in the canvas space, and mapped back using the camera homographies to form time-varying noise images $Z_t$. The final mask inputs are $M_t^i' = M_t^i * (1 - M_t^i)Z_t$. This is a similar approach to Lu, et al.~\cite{lu2020layered}, but in our case the texture is fixed. 

\subsection{Background Layer}

As the background is assumed to be static, we treat it specially. The network input for the background layer is the fixed noise texture $\Bar{Z}$, and the output is a fixed background RGB image $\Bar{C}^0$ in canvas space. For composition, this background image is sampled using the camera homographies to form time-varying background layers $C_t^0$. 

Due to camera effects such as exposure changes, vignetting, and radial distortion, even a stationary background usually changes in appearance slightly from frame to frame. If the background is assumed to be entirely static, these subtle shifts in appearance will be captured by the omnimatte and contaminate it. 

To handle deviations from the static background assumption, we note that effects caused by the camera, such as vignetting and exposure, tend to have low spatial and temporal frequency relative to the subject's effects. Camera effects can be safely captured by applying a coarse \emph{refinement warp} to the background layer. The refinement warp consists of a grid-based warp and a grid-based brightness adjustment to the background color map $C^0_t$ at pixel $\mathbf{x}$:

\begin{equation}
    C^0_t'(\mathbf{x}) = C^0_t(\mathbf{G_w}[t,x_v,x_u]) \cdot \mathbf{G_b}[t,x_v,x_u]
\end{equation}

where $\mathbf{G_w}$ is a $n/10 \times 4 \times 7 \times 2$ grid of offset vectors, $\mathbf{G_b}$ is a $n/10\times 4 \times 7$ grid of brightness coefficients, $n$ is the number of frames in the video, and $[\cdot,\cdot,\cdot]$ denotes trilinear filtering. The values of $\mathbf{G_w}$ and $\mathbf{G_b}$ are optimized together with the network parameters. 
